Arabic Dialect Identification in the Wild

We present QADI, an automatically collected dataset of tweets belonging to a wide range of country-level Arabic dialects -covering 18 different countries in the Middle East and North Africa region. Our method for building this dataset relies on applying multiple filters to identify users who belong to different countries based on their account descriptions and to eliminate tweets that are either written in Modern Standard Arabic or contain inappropriate language. The resultant dataset contains 540k tweets from 2,525 users who are evenly distributed across 18 Arab countries. Using intrinsic evaluation, we show that the labels of a set of randomly selected tweets are 91.5% accurate. For extrinsic evaluation, we are able to build effective country-level dialect identification on tweets with a macro-averaged F1-score of 60.6% across 18 classes.

==> random.tex <==
\section{Random}
XXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXXX
In this work, we attempt to build a resource that is generic enough and with high coverage. Previous attempt to build a suitable resources
focused on users profiling through their tweets \cite{bouamor-etal-2019-madar}. While in the current work we aim at providing a resource that would be used further than Social Media as we attempt to remove salient features related to Social media such as Hashtags (NOOOO), Mentions, Emoticons and URL. This will result in elements that are purely textual and transcend social media to cover other genera such as email, blogs, reports and other written artifacts. This will make it more suitable for other tasks such as user profiling, language and dialect identification among other NLP tasks. Our contributions in this paper are manifold:\newline
\begin{enumerate}
\item We provide a list of Twitter users from 18 Arab countries in the MENA region (a total of 3429 accounts, average = 190 per country) BUT THIS IS BEFORE FILTRATION. We need to compare with Wajdi's work about author profiling. how many accounts in his paper?\newline

We provide a list of 540K dialectal tweets from these users (average of 30k tweets for each country). Geographical distribution of the dialects are shown in Figure \ref{dialects}.\footnote{ https://mapchart.net/world.html}
\item We create a new testset of 200 tweets per country that are manually annotated by native speakers (a total of XXX tweets after manual verification by native speakers, also 200 for MSA)
\item We perform extensive comparisons with MADAR Shared Task~\cite{bouamor-etal-2019-madar} data, which is regarded as the most diverse resource for Arabic dialect ID to date. We show that our data is more balanced and representative while maintaining similar level of diversity.
\item We show that harvesting user description can greatly help in collecting high accurate dialectal tweets and potentially in other tasks as well, ex. author profiling and social studies.
\item In our data analysis, we show experimentally how close or far dialects from each other using the collected data, ex: dialects spoken in SY and LB are close to each other, and JO and PL dialects are close to each other and close to SY and LB dialects more than EG dialect, etc. We also identify most common dialectal words for each country. Accuracy of these lists can be enhanced by manual filtration by native speakers.
\item We extensively experiment on different machine learning models, deep neural networks (DNNS) and contextual embeddings to perform automated dialect ID. We train and evaluate our models on our proposed dataset and MADAR shared task dataset.

\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.4, frame]{coling2020/figures/dialectmap.png} 
\caption{Dialects in MENA region. HAMDY: I prefer  \url{https://sblanguagemaps.files.wordpress.com/2014/06/arabic-dialects2.png}}
\label{dialects}
\end{center}
\end{figure}


\end{enumerate}
\textbf{Note}:
We use ISO 3166-1 alpha-2 codes for country codes\footnote{\url{https://en.wikipedia.org/wiki/ISO_3166-1_alpha-2}}, and we sort Arab countries by their population\footnote{\url{https://www.worldometers.info/world-population/population-by-country/}} ex: EG for Egypt, DZ for Algeria, etc.  in all parts of the paper.\\

FIXME: We need to show a map for the countries (dialects) because this helps when we discuss the geographical closeness between dialects in the hierarchical clustering.
how about this map \url{https://sblanguagemaps.files.wordpress.com/2014/06/arabic-dialects2.png} because is shows that it's hard to distinguish between SY and LB also between JO and PL?


% \section{Data Description}

% To build our dataset, we obtained a collection of Arabic tweets that was obtained using the Twitter \textcolor{red}{streaming?} API, where we set the language filter to Arabic ("lang:ar"), during March and April 2018. In all, we collection contains 25M tweets from which we identified the profile information of all the users who authored the tweets. We applied three filters on user profile to ascertain accounts that are from specific countries that tweet mostly in dialectal Arabic and do not promote inappropriate content, such as vulgar or sexually explicit content.  

% The first filter attempted to determined that an account originated from a specific country using user self-disclosure, where users would specify specific country or city name or nationality in the user profile description.  Table \ref{tab:ExamplesOfSelfDeclaration} shows some examples of such self-disclosures.  To ascertain country membership we used a gazetteer that includes:
% \begin{itemize}
%     \item all Arabic countries names written in either Arabic, English, or French\footnote{French is widely used in the Maghreb region.} such as \<المغرب>
%     (Almgrb -- Morocco), Morocco, and Maroc.
%     \item the names of major cities in these countries in both Arabic and English as specified in Wikipedia\footnote{\url{https://en.wikipedia.org/wiki/List_of_countries_by_largest_and_second_largest_cities}} such as \<القدس> 
%     (Alqds -- Jerusalem) and \<وهران> 
%     (whrAn -- Oran, Algeria).
%     \item adjectives specifiying all nationalities in both masculine and feminine forms with and without the definite article \<ال> (Al -- the) such as 
%     \<عراقي> (ErAqy - Iraqi (m.)), \<عراقية> (ErAqyp - Iraqi (f.)), and 
%     \<العراقي> (AlErAqy - the Iraqi (m.)).
% \end{itemize}
% In all the gazetteer contained 200 items in total.  

% The second filter checks if the account mainly tweets in either dialectal Arabic or MSA.  Since Arabic users switch between MSA and dialectal Arabic and we were interested in strictly dialectal tweets, we sought to filter out MSA tweets. There are multiple ways to distinguish between dialectal and MSA text.  One such method involves using a list of strictly dialectal words ~\cite{Darwish:2014:verifiably}.  However, constructing such lists across multiple dialects can be challenging.  We opted to train a text classifier using crudely labeled tweet set.  Specifically, given 50 million tweets that we collected between March and September 2018, we assumed that tweets containing the MSA relative pronouns \<الذي، الذى، التي، التى، الذين> 
% ("Al*y, Al*Y, Alty, AltY, Al*yn" - who/that in masculine, feminine and plural forms) as MSA, and those containing the dialectal relative pronoun \<اللي، اللى>  
% ("Ally, AllY" -- who/that) as dialectal.  The dialectal relative pronoun \<اللي>  
% is present in most Arabic dialects.  In doing so, we extracted 3.09M MSA tweets and 3.17M dialectal tweets. For these tweets, we replaced user mentions with @USER, digits to NUM, emojis to EMOJI, URLs to URL, and relative pronouns to RELATIVE. In doing so, we eliminated Twitter Twitter-specific features, which are not linguistic in nature, and the relative pronouns, which we used to construct the training set. We set aside 10k MSA and dialectal tweets for testing.  We trained a fastText text classifier, which deep-leaning based classifier, using character n-grams ranging in length between 3 and 6 grams. We tested the heldout test set, and the accuracy of distinguishing between MSA and dialectal Arabic was 98\%.  Using this classifier, we classified the tweets of the users.  We retained users, where at least 50\% of their tweets were dialectal.

% The third filter removed users who were mostly tweeting vulgar, sexually explicit, or pornographic tweets.  To filter out these users.  For filtration, we used the obscene word list generated by Mubarak et al. \citename{mubarak2017abusive}, which contains 288 words and 127 hashtags.  We removed users if more than 50\% of their tweets contained vulgar words.

% After the three filtration steps, we ranked users based on the number of followers in descending order for each country.  We asked an annotator to inspect all the profiles from each country starting from the top of the lists to identify the first 200 profiles that indeed belonged to individual countries. The annotator further skipped profiles if: they mostly contained poetry, particularly Bedouin poetry; the person declares that (s)he is from more than one place (e.g. Palestinian raised in Egypt); or they were too similar to previously selected profiles, which typically resulted from propaganda accounts that generally spread very similar content. In all, we identified 3,430 users from 18 different Arabic speaking countries in the MENA region (190 accounts per country on the average). Further, we used the aforementioned MSA/dialectal classifier to filter out MSA tweets from their timelines.  In doing so, we identified 540k dialectal tweets that are balanced across the 18 countries (approximately 30k tweets per country).

% %We used fastText classifier to estimate quality of our approach by extracting random 20k tweets (10k for each class) and train on the remaining tweets. We replaced the relative particles with a dummy token in MSA and DA tweets, also in training and testing sets, such that we allow the classifier to depend on other contextual information in the tweets to increase its generalization and robustness.

% % While it's hard to distinguish dialects from each other, it's much easier to decide whether a tweet is written in DA or MSA. This can be done using different methods, e.g. using lists of common dialectal and MSA words, or by collecting tweets from accounts which mainly post MSA tweets like accounts for news agencies, official accounts for governments and embassies, etc. The problems with the aforementioned methods are: they need manual effort to create these lists of dialectal and MSA words also these Twitter accounts; and the collection of tweets will be biased towards specific dialects or genres according to the data used to filter tweets. We opted to use a very simple yet efficient method to collect DA and MSA tweets without giving any preference to any dialect or genre. The details of our method are described as follows: \newline

% % During the period between 2018-03-04 and 2019-09-26, we collected approx. 50M Arabic tweets using Twitter API and "lang:ar". If a tweet has any of the MSA relative particles \<الذي، الذى، التي، التى، الذين> ("Al*y, Al*Y, Alty, AltY, Al*yn" - who/that in masculine, feminine and plural forms), the tweet was labeled as MSA. And if a tweet has any of the dialectal variations \<اللي، اللى> ("Ally, AllY"), it was labeled as DA\footnote{We also used these prefixes for MSA: \<و، ف، ب، ل، ك> ("w, f, b, l, k" - and, so, in, for, as). For DA, we used the following prefixes: \<و، ب، ل> ("w, b, l" - and, in, for)}. These groups of relative particles are used exclusively in either MSA or DA, and they are generic and used across all dialects without any preference to specific genre or dialect. We used the masculine, feminine and plural forms for MSA and different dialectal writings to have a wider coverage of styles and dialects.\newline

% % By applying the aforementioned filters, we extracted 3.09M MSA tweets and 3.17M DA tweets. These tweets were normalized by converting user mentions to @USER, digits to NUM, emojis to EMOJI, URLs to URL, and new lines in the middle of tweets to NEWLINE. These normalization steps allow for more generalization to distinguish MSA from DA classes without depending on Twitter-specific information like mentioning some user accounts. We used fastText classifier to estimate quality of our approach by extracting random 20k tweets (10k for each class) and train on the remaining tweets. We replaced the relative particles with a dummy token in MSA and DA tweets, also in training and testing sets, such that we allow the classifier to depend on other contextual information in the tweets to increase its generalization and robustness.

% % We got the list of Arabic countries and major cities from Wikipedia\footnote{\url{www.XXX.YYY}} in Arabic, English (and French\footnote{French is widely used in the Maghreb region.}), ex: for , we have the following entries in addition to Arabic and English names: Maroc, \<الرباط>, Rabat, \<الدار البيضاء>, and Casablanca. Also, we created a list of adjectives for nationalities of these countries in masculine and feminine forms, ex: \<عراقي> ("ErAqy" - Iraqi (m.)), \<عراقية> ("ErAqyp" - Iraqi (f.), and their forms after adding the definite article \<ال> ("Al" - the). We ended up with a list of 200+ words that we will use to initially map tweets from users to one of Arab countries. We call this list "CountryNames".



% of unique users who posted any of those tweets. If we found any of the CountryNames words in either username or user description\footnote{Only the top 5 words are considered}, we extracted those accounts and all their profile information. We sorted this initial list of users based on their followers counts such that the most popular accounts come first. The intuition behind this is that popular accounts potentially post many tweets such that when we get their history of tweets, we would find larger number of dialectal tweets. 

% During this manual selection of users for potential collection of dialectal tweets, we considered the following: \\
% \begin{itemize}
% \item Exclude users who potentially post tweets in dialects that are different than their declared country, for example we exclude official organizations, political figures, Arabic teachers, etc. because they will not post much dialectal tweets,
% \item Exclude users who potentially post inappropriate tweets (e.g. post adult-content or vulgar tweets),
% \item Try to have diverse users in terms of gender (males and females), political ideologies, religious, etc.
% \item Take same number of users from each country such that we don't give any preference to specific countries.
% Except 2 countries, namely MA and TN, we initially set the number of users for each country to be 200. Complete statistics of users are listed in Table XXX.\newline
% \end{itemize}



HAMDY: XXXXXX\\
Contributions:
- largest dialectal tweets (balanced and divers)
- 3000+ user profiles (originally 200 from each country before filtration, and we ended up with xxx users)
- testset of dialectal tweets (200 per country) verified by natives speakers from 18 countries
- generic methodology for collecting dialectal tweets only from user profiles and filtering dialectal tweets from MSA tweets from the tweet history of those users
- new SOTA on madar testset at user-level and we show that SVM char-level is better than other classifiers (including BERT) in dialect classification task
- extract the most common distinguishing words (valence score) for each dialect
- show the closeness of dialects that are spoken in geographically-closed countries (for ex: north Levant (SY and LB) and south Levant (JO and PL)) which explains which dialects are hard to identify.\newline



User location was used in collecting dialectal tweets (our previous work).. harvesting user profile info was not utilized much...\\
Users express their identity, nationality, etc.. examples in Figure \ref{userDescrExamples}.

\begin{figure}[h]
\begin{center}
\includegraphics[scale=0.8, frame]{coling2020/figures/userDescrExamples.png} 
\caption{User Description Examples}
\label{userDescrExamples}
\end{center}
\end{figure}


%\url{www.ar.wikipedia.org/wiki/قائممة_المدن_الكبرى_حسب_الدولة



Note:
We assume that normally users post tweets in either their local dialect or in MSA. For each country, we ended up with users who specify their nationality in their profiles and their history of tweets that are supposed to be either in their dialects or in MSA. In the next section, we show how to extract only dialectal tweets from a corpus contains also MSA tweets.\\

points:\\
1. User description is not yet utilized to end\\
2. Many users identify themselves in their profile according to their nationality, religion, political ideology, etc. in terms of a country flag, image, or textual description.\\
3. Sort user according to followers count (most probably they will post many tweets)\\
4. Try to balance between male and female users, from different religions and ideologies\\
5. Ignore users who probably post tweets in other than their own dialect (ex: Arabic teachers, poets, political figures, etc.) in addition to users who describe in their profile that they will post inappropriate tweets (ex: adult-content or vulgar words, etc.)\newline
6. When we took the same number of users from each country (then collect their history of tweets and exclude MSA), we try to have balanced data and not to give any preference to any country. If we just collect random Arabic tweets, majority of them will be from Gulf countries (SA, KW, AE..) (cite previous work if you wish) and will end up with a totally skewed data.\newline
7. We have tweets from 18 Arab countries as we didn't find much users or Arabic tweets from 4 of the Arab countries, namely: Mauritania, Somalia, Dijbouti, and Comoros.

We need to mention that during our collection, we applied the following preprocessing steps to make classifiers rely on contextual data not on other Twitter-specific data (ex: mentioning of some users or replies to some users as a signal to detect country, for example if a tweet retweets a news from $@$alriyadh newspapers, this may help the classifier to guess the dialect to be from SA):
all user mentions are mapped to $@$USER, all URLs are mapped to URL, emojis are mapped to EMOJI, all numbers are mapped to NUM, and new lines in the middle of the text to NEWLINE.



\subsection{Distinguish dialects from MSA}
Hamdy: XXXXXX\newline
% While it's hard to distinguish dialects from each other, it's much easier to decide whether a tweet is written in DA or MSA. This can be done using different methods, e.g. using lists of common dialectal and MSA words, or by collecting tweets from accounts which mainly post MSA tweets like accounts for news agencies, official accounts for governments and embassies, etc. The problems with the aforementioned methods are: they need manual effort to create these lists of dialectal and MSA words also these Twitter accounts; and the collection of tweets will be biased towards specific dialects or genres according to the data used to filter tweets. We opted to use a very simple yet efficient method to collect DA and MSA tweets without giving any preference to any dialect or genre. The details of our method are described as follows: \newline

% During the period between 2018-03-04 and 2019-09-26, we collected approx. 50M Arabic tweets using Twitter API and "lang:ar". If a tweet has any of the MSA relative particles \<الذي، الذى، التي، التى، الذين> ("Al*y, Al*Y, Alty, AltY, Al*yn" - who/that in masculine, feminine and plural forms), the tweet was labeled as MSA. And if a tweet has any of the dialectal variations \<اللي، اللى> ("Ally, AllY"), it was labeled as DA\footnote{We also used these prefixes for MSA: \<و، ف، ب، ل، ك> ("w, f, b, l, k" - and, so, in, for, as). For DA, we used the following prefixes: \<و، ب، ل> ("w, b, l" - and, in, for)}. These groups of relative particles are used exclusively in either MSA or DA, and they are generic and used across all dialects without any preference to specific genre or dialect. We used the masculine, feminine and plural forms for MSA and different dialectal writings to have a wider coverage of styles and dialects.\newline

% By applying the aforementioned filters, we extracted 3.09M MSA tweets and 3.17M DA tweets. These tweets were normalized by converting user mentions to @USER, digits to NUM, emojis to EMOJI, URLs to URL, and new lines in the middle of tweets to NEWLINE. These normalization steps allow for more generalization to distinguish MSA from DA classes without depending on Twitter-specific information like mentioning some user accounts. We used fastText classifier to estimate quality of our approach by extracting random 20k tweets (10k for each class) and train on the remaining tweets. We replaced the relative particles with a dummy token in MSA and DA tweets, also in training and testing sets, such that we allow the classifier to depend on other contextual information in the tweets to increase its generalization and robustness.

The classification accuracy was 98\% using the following settings: apply char-level classification between 3 and 6 char-ngrams, dimension of word vector is 100, learning rate = 0.05, and it was running for 50 epochs. This shows that distinguishing MSA from DA can easily achieve high accuracy using our simple method for extraction and classification. \newline

FIXME:
fastText model was used to judge whether a tweet is dialectal or not. We assume that normally users write tweets either in their dialects or MSA, and if the classifier judges that a tweet is in DA, we will assume that the tweet is written in the dialect of the user based on their profile description. To extract most accurate tweets, we considered only tweets that are classified as DA by the classifier with a confidence level of 98\% or above.








\begin{figure*}[h]
\begin{center}
%\fbox{\parbox{6cm}{
%This is a figure with a caption.}}
\includegraphics[scale=0.6]{figures/stat.png} 
\caption{We need to add stats graph like this, we can show that MADAR data is totally imbalanced, 40\% from SA, also we have larger number of accounts. WARNING: take final numbers from QADI\_train.txt + 200 tweets per country for testing. NOTE: We can divide final tweets / original tweets to show percentage, if the ratio is small, this means that the classifier was not confident in many cases, i.e. the dialect is more close to MSA}
\label{fig.1}
\end{center}
\end{figure*}



\begin{figure*}[h]
\begin{center}
%\fbox{\parbox{6cm}{
%This is a figure with a caption.}}
\includegraphics[scale=0.6]{figures/account-dist.png} 
\caption{Dialect ID bar chart}
\label{dialectID-bar}
\end{center}
\end{figure*}

\begin{figure*}[h]
\begin{center}
%\fbox{\parbox{6cm}{
%This is a figure with a caption.}}
\includegraphics[scale=0.6]{figures/QADI_tweets_distribution_piechart.pdf} 
\caption{QADI data distribution per country}
\label{fig.1}
\end{center}
\end{figure*}










